The Burden of Risk Aversion in Mean-Risk Selfish Routing

Considering congestion games with uncertain delays, we compute the inefficiency introduced in network routing by risk-averse agents. At equilibrium, agents may select paths that do not minimize the expected latency so as to obtain lower variability. A social planner, who is likely to be more risk neutral than agents because it operates at a longer time-scale, quantifies social cost with the total expected delay along routes. From that perspective, agents may make suboptimal decisions that degrade long-term quality. We define the {\em price of risk aversion} (PRA) as the worst-case ratio of the social cost at a risk-averse Wardrop equilibrium to that where agents are risk-neutral. For networks with general delay functions and a single source-sink pair, we show that the PRA depends linearly on the agents' risk tolerance and on the degree of variability present in the network. In contrast to the {\em price of anarchy}, in general the PRA increases when the network gets larger but it does not depend on the shape of the delay functions. To get this result we rely on a combinatorial proof that employs alternating paths that are reminiscent of those used in max-flow algorithms. For {\em series-parallel} (SP) graphs, the PRA becomes independent of the network topology and its size. As a result of independent interest, we prove that for SP networks with deterministic delays, Wardrop equilibria {\em maximize} the shortest-path objective among all feasible flows.

==> braess-mean-stdev.tex <==
%auto-ignore
\section{PRA in the Braess Network in the Mean-Stdev Model}\label{sec:braess-mean-stdev}

In this section we specialize our results to the Braess paradox network with
a single OD and unit demand. Suppose that the top path $p$ is composed of
edges $a$ and $b$, the bottom path $q$ is composed of edges $c$ and $d$, and
the zigzag path $r$ is composed of edges $a$, $e$, and $d$.

We first restate Lemma~\ref{boundBraess} (corresponding to Lemma~\ref{boundBraess-meanvar} in the mean-var model) that we use in our subsequent proofs. 

\begin{lemma}\label{boundBraess-meanstdev}
For a general Braess network, if $\sigma_r$ is not largest and $x_r > 0$, then
the cost at a RAWE
$$C^0(x) \le (1+\gamma\kappa) (\ell_c(x_c)+\ell_b(x_b))-\ell_e(x_e).$$
\end{lemma}
\begin{proof}
First, we prove that under the assumptions of the lemma,
$\sigma_p + \sigma_q -\sigma_r\le \sigma_b+\sigma_c$.
Indeed, that inequality is equivalent to
\begin{align*}
\sqrt{\sigma_a^2+\sigma_b^2}+ \sqrt{\sigma_c^2+\sigma_d^2} \le & \sigma_b+\sigma_c+\sqrt{\sigma_a^2+\sigma_e^2+\sigma_d^2} \Leftrightarrow\\
2\sqrt{(\sigma_a^2+\sigma_b^2)(\sigma_c^2+\sigma_d^2)}\le&2\sigma_b\sigma_c+\sigma_e^2+2(\sigma_b+\sigma_c)\sqrt{\sigma_a^2+\sigma_e^2+\sigma_d^2}\Leftrightarrow\\
\sigma_a^2\sigma_d^2\le& \frac{\sigma_e^4}{4}+\sigma_b\sigma_c\sigma_e^2+\sigma_a^2\sigma_b^2+\sigma_c^2\sigma_d^2+2\sigma_b\sigma_c(\sigma_a^2+\sigma_e^2+\sigma_d^2)+\nonumber\\
&\quad \sigma_e^2(\sigma_b^2+\sigma_c^2)+(2\sigma_b\sigma_c+\sigma_e^2)(\sigma_b+\sigma_c)\sqrt{\sigma_a^2+\sigma_e^2+\sigma_d^2}
\end{align*}
If $\sigma_p\ge\sigma_r$, the last inequality holds because
$\sigma_a^2+\sigma_b^2\ge \sigma_a^2+\sigma_e^2+\sigma_d^2$, from where
$\sigma_b\ge \sigma_d$. The case of $\sigma_q\ge\sigma_r$ is similar.


Since $x_r > 0$, we have that 
\begin{eqnarray}%\label{eq:d}
&& \ell_r(x) + \gamma \sigma_r \leq \ell_p(x) + \gamma \sigma_p \nonumber \\
\Leftrightarrow && \ell_a(x) + \ell_e(x) + \ell_d(x) \leq \ell_a(x) + \ell_b(x) + \gamma (\sigma_p-\sigma_r) \nonumber \\
\Leftrightarrow &&  \ell_d(x) \leq \ell_b(x) -\ell_e(x) + \gamma (\sigma_p-\sigma_r). \label{eq:d1}
\end{eqnarray}
Similarly, 
\begin{eqnarray}
&& \ell_r(x) + \gamma \sigma_r \leq \ell_q(x) + \gamma \sigma_q \nonumber \\
\Leftrightarrow && \ell_a(x) + \ell_e(x) + \ell_d(x) \leq \ell_c(x) + \ell_d(x) + \gamma (\sigma_q-\sigma_r) \nonumber \\
\Leftrightarrow &&  \ell_a(x) \leq \ell_c(x) -\ell_e(x) + \gamma (\sigma_q-\sigma_r). \label{eq:a1}
\end{eqnarray}

Using the previous inequalities,
\begin{align*}
C^0(x) = & \sum_{\pi} x_{\pi} \ell_{\pi}(x) \\
\leq & \sum_{\pi} x_{\pi} (\ell_r(x) + \gamma\sigma_r - \gamma\sigma_{\pi}) 
\qquad \mbox{ because either } x_{\pi} = 0 \mbox{ or } \ell_{\pi}(x) + \gamma\sigma_{\pi} \leq \ell_r(x) + \gamma\sigma_r \\
= & \ell_a(x) + \ell_e(x) + \ell_d(x) +\gamma\sigma_r - \gamma\sum_{\pi} x_{\pi}\sigma_{\pi}  \\
\leq & \ell_a(x) + \ell_e(x) + \ell_d(x) +\gamma\sigma_r \\
\leq & \ell_c(x) -\ell_e(x)+ \gamma(\sigma_q-\sigma_r)+ \ell_e(x) + \ell_b(x) -\ell_e(x)+ \gamma(\sigma_p-\sigma_r) +\gamma\sigma_r \qquad\mbox{ by Eq.(\ref{eq:d1})-(\ref{eq:a1})}\\
= & \ell_c(x) + \ell_b(x) -\ell_e(x)+\gamma(\sigma_p + \sigma_q -\sigma_r)\\
\le & \ell_c(x) + \ell_b(x) -\ell_e(x)+\gamma(\sigma_b+\sigma_c)\\
\le & (1+\gamma\kappa) (\ell_c(x_c)+\ell_b(x_b))-\ell_e(x_e), 
\end{align*}
where the last inequality follows from the coefficient of variability constraint  $\sigma \leq \kappa \ell(x)$ for the corresponding edges. 
\end{proof}



\begin{theorem}
In an asymmetric Braess network:
\begin{enumerate}
\item If $x_p < z_p$ and $x_q < z_q$, then $C^0(x) \leq (1+2\gamma\kappa) C^0(z).$
\item Otherwise, $C^0(x) \leq (1+\gamma\kappa) C^0(z).$
\end{enumerate}
\end{theorem}
%
\begin{proof}
{\bf Case (1.1): $x_p < z_p$ and $x_q < z_q$ and $\sigma_r$ is not largest}.  Then, $x_r > z_r$, so $x_r > 0$. Also, 
\begin{eqnarray*}
x_c &=& x_q < z_q = z_c \\
x_b &=& x_p < z_p = z_b \\
x_e &=& 1-x_p-x_q > 1-z_p-z_q = z_e.
\end{eqnarray*}
%
Then, we have:
\begin{eqnarray*}
C^0(x) &\leq& (1+\kappa\gamma)\left( \ell_c(x_c) + \ell_b(x_b) \right) - \ell_e(x_e) \qquad \mbox{ by Lemma~\ref{boundBraess-meanstdev}} \\
&\leq& (1+\kappa\gamma)\left( \ell_c(z_c) + \ell_b(z_b) \right) - \ell_e(z_e) \qquad \mbox{ by the inequalities above} \\
&=& \ell_c(z_c) -\ell_e(z_e) +\ell_b(z_b)  + \gamma\kappa \left( \ell_c(z_c) + \ell_b(z_b) \right) \\
&\leq& \ell_p(z) + \gamma\kappa \left( \ell_c(z_c) + \ell_b(z_b) \right) \qquad \mbox{ since $z_q > 0$ and hence } \ell_c(z_c)-\ell_e(z_e) \leq \ell_a(z_a) \\
&=& C^0(z) + \gamma\kappa \left( \ell_c(z_c) + \ell_b(z_b) \right) \qquad \mbox{ since $z_p > 0$ and hence } \ell_p(z) = C^0(z) \\
&\leq& C^0(z) + 2\gamma\kappa C^0(z) \qquad \mbox{ because } \ell_c(z_c) \leq \ell_q(z) = C^0(z) \\
&=& (1+2\gamma\kappa) C^0(z). 
\end{eqnarray*}

{\bf Case (1.2): $x_p < z_p$ and $x_q < z_q$ and $\sigma_r = \max(\sigma_p,\sigma_q,\sigma_r)$}. THIS IS THE ONLY CASE LEFT TO PROVE. 

{\bf Case (2.1): $x_p \geq z_p$ and $x_q \geq z_q$}.  
\begin{eqnarray*}
x_a &\leq& z_a = 1-z_q \\
x_e &\leq& z_e = 1-z_p-z_q \\
x_d &\leq& z_d = 1-z_p.
\end{eqnarray*}
%
If $z_r > 0$, then  
\begin{eqnarray*}
C^0(x) &\leq& (1+\kappa\gamma)\left( \ell_a(x_a) + \ell_e(x_e) + \ell_d(x_d) \right) \qquad \mbox{ by Lemma~\ref{thm-UBcostRAWE-var}} \\
&\leq& (1+\kappa\gamma)\left( \ell_a(z_a) + \ell_e(z_e) + \ell_d(z_d) \right) \qquad \mbox{ by the above inequalities} \\
&=& (1+\kappa\gamma)\ell_r(z) \\
&=& (1+\kappa\gamma) C^0(z) \qquad \mbox{ since } z_r > 0 \mbox{ so } C^0(z)=\ell_r(z).
\end{eqnarray*}
%
Else, when $z_r = 0$, then $x_r \geq z_r$.  Then $x \geq z$ as vectors, but their coordinates both sum up to 1, therefore $x = z$ and hence $C^0(x)=C^0(z)$.

%
{\bf Case (2.2): $x_p \geq z_p$ and $x_q < z_q$}.  Then, $z_q > 0$ and 
%
\begin{eqnarray*}
x_c &=& x_q < z_q = z_c \\
x_d &=& 1-x_p \leq 1-z_p = z_d.
\end{eqnarray*}
%
Hence, 
\begin{eqnarray*}
C^0(x) &\leq& (1+\kappa\gamma)\left( \ell_c(x_c) + \ell_d(x_d) \right) \qquad \mbox{ by Lemma~\ref{thm-UBcostRAWE-var}} \\
&\leq& (1+\kappa\gamma)\left( \ell_c(z_c) + \ell_d(z_d) \right) \qquad \mbox{ by the above inequalities} \\
&=& (1+\kappa\gamma) C^0(z) \qquad \mbox{ since } z_q > 0 \mbox{ so } C^0(z)=\ell_q(z).
\end{eqnarray*}

{\bf Case (2.3): $x_p < z_p$ and $x_q \geq z_q$}.  This case is analogous to Case (2.2).  

\end{proof}


==> equilibrium.tex <==
%auto-ignore
%%%%%%%%%%%%
\subsection{Example}

Next, we see an example where the price of risk aversion is even higher than $1+\kappa\gamma$, in this case it can get up to $1+2\kappa\gamma,$ for a particular value of $\kappa\gamma$.

\begin{example}\label{ex:braess}
Consider the symmetric Braess network instance in Figure~\ref{fig:pra-counterexample} with latencies $\ell_a(x) = \ell_d(x) = \alpha x$, $\ell_b(x) = \ell_c(x) = 1$ and $\ell_e(x) = \beta + v$, and let
the standard deviations (respectively, variances in the mean-variance model) of edges be $\sigma_a=\sigma_d=\sigma_e=0$ and $\sigma_b = \sigma_c = v$.  Further, set $\gamma = 1$, $\kappa = v$ so that $\kappa\gamma = v$.  Note that this satisfies the definition of coefficient of variability, for which we need $\sigma \leq \kappa$ (respectively, $v \leq \kappa$).

%
\begin{figure}
\begin{center}
\psfrag{1}[c][c]{\footnotesize$(1,v)$}
\psfrag{z}[l][l]{\footnotesize$(\beta+v,0)$}
\psfrag{d}[c][c]{\footnotesize$1$}
\psfrag{x}[c][c]{\footnotesize$(\alpha x,0)$}
\includegraphics[height=30mm]{braess}
\end{center}
%\centering\includegraphics[width=2.5in]{./figures/mean-var-1plus2kappagamma-counterexample}
\caption{Example with $PRA \rightarrow 1+2\kappa\gamma$ in the mean-var model. Edges are labeled with (mean,variance) pairs and we assume $v = \kappa$ and $\gamma = 1$.}\label{fig:pra-counterexample}
\end{figure}
%


%%%%%
First, we compute the risk-averse equilibrium. Denote the equilibrium flow on paths $p$ and $q$ by $x_p = x_q = x$. We can check that at equilibrium all path costs are equal (that is, the equilibrium is always an interior one or behaves like an interior one.)  Equating risk-averse costs of the top and zigzag paths gives:
%
\begin{eqnarray*}
&& \ell_a(x_a) + \ell_b(x_b) + \gamma v_p = \ell_a(x_a) + \ell_e(x_e) + \ell_a(x_a) \\
\Leftrightarrow && \ell_b(x_b) + \gamma v_p = \ell_a(x_a) + \ell_e(x_e) \\
\Leftrightarrow && 1 + v = \alpha(1-x) + \beta + v \\
\Leftrightarrow && 1 + \alpha x = \alpha + \beta  \\
\end{eqnarray*}

We will ensure that $x = 0$ (that is, $x_r = 1$, the zigzag path carries all flow) is an equilibrium.  From above, $\alpha + \beta = 1$.  From here on, we set $\beta = 1 - \alpha$. With this, the path costs are:

\begin{eqnarray*}
C_p(x) = C_q(x) &=& \alpha + v + 1 \\
C_r(x) &=& 2\alpha + \beta + v
\end{eqnarray*}

Therefore, the cost of the risk-averse equilibrium is

\begin{eqnarray*}
C^0(x) = \alpha + v + 1 = \ell_r(x).
\end{eqnarray*}
%%%

Next, let us compute the risk-neutral equilibrium. Denote $z_p = z_q = z$.  Then, $z_a = 1 - z_q = 1-z$ and therefore
%
\begin{eqnarray*}
\ell_p(z) &=& \ell_a(z_a) + \ell_b(z_b) = \alpha(1-z) + 1 \\
\ell_r(z) &=& \ell_a(z_a) + \ell_e(z_e) + \ell_a(z_a) = 2\alpha(1-z) + 1-\alpha + v.
\end{eqnarray*}
%
Assuming interior risk-neutral equilibrium, we have:
%
\begin{eqnarray*}
&& \ell_a(z_a) + \ell_b(z_b) = \ell_a(z_a) + \ell_e(z_e) + \ell_a(z_a) \\
\Leftrightarrow && \alpha(1-z) + 1 = 2\alpha(1-z) + 1-\alpha + v \\
\Leftrightarrow && 0 = \alpha(1-z) -\alpha + v \\
\Leftrightarrow && \alpha-v = \alpha(1-z) \\
\Leftrightarrow && 1-z = \frac{\alpha-v}{\alpha} = 1 - \frac{v}{\alpha} \\
\Leftrightarrow && z = \frac{v}{\alpha} \in [0,\frac{1}{2}] \\
\end{eqnarray*}
%
Therefore, $\frac{v}{\alpha} \leq \frac{1}{2}$, or equivalently $\alpha \geq 2 v$.

The cost of the risk-neutral equilibrium is
%
\begin{eqnarray*}
C^0(z) = \ell_p(z) = \alpha \frac{\alpha-v}{\alpha} + 1 = \alpha - v + 1.
\end{eqnarray*}
%
Therefore, the PRA is
%
\begin{eqnarray*}
\frac{C^0(x)}{C^0(z)} = \frac{\alpha+1+v}{\alpha+1-v} = 1+f v,
\end{eqnarray*}
%
where
%
\begin{eqnarray*}
&& fv = \frac{\alpha+1+v}{\alpha+1-v} - 1 = \frac{\alpha+1+v-\alpha-1+v}{\alpha+1-v}
   = \frac{2v}{\alpha+1-v} \\
\Leftrightarrow && f = \frac{2}{\alpha+1-v} \rightarrow 2 \mbox{  as } v\rightarrow 0,
\end{eqnarray*}
%
where $\alpha=2v$ is the worst case for the factor $f$.
This concludes the matching lower PRA bound.
\end{example}

Actually the worst-case instance is really the one shown in
Figure~\ref{fig:pra-counterexample2} after we replace all coefficients we got
in the previous paragraphs. For this instance the RNWE is $z=(1/2,1/2,0)$
with $C_0(z)=l_P(z)=1+v$, and the RAWE is $x=(0,0,1)$ with
$C_0(x)=l_r(x)=3v+1$. Dividing, we get that the
$$\text{PRA}=\frac{3v+1}{v+1}.$$
This works for $v\le 1$. Hence, the worst-case bound of $1+f\kappa\gamma$ is
achieved when $v=\kappa\to 0$ and in that case $f\to 2$, showing that the
upper bound of the form $1+f\kappa\gamma$ is tight for $f=2$. With this we
know that the PRA is between $1+\kappa\gamma$ and $1+2\kappa\gamma$ but we
don't know the exact PRA.

\begin{figure}[h]
\begin{center}
\psfrag{1}[c][c]{\footnotesize$(1,v)$}
\psfrag{z}[l][l]{\footnotesize$(1-v,0)$}
\psfrag{d}[c][c]{\footnotesize$1$}
\psfrag{x}[c][c]{\footnotesize$(2vx,0)$}
\includegraphics[height=30mm]{braess}
\end{center}
%\centering\includegraphics[width=2.5in]{./figures/mean-var-1plus2kappagamma-counterexample}
\caption{Example with $PRA \rightarrow 1+2\kappa\gamma$ in the mean-var model. Edges are labeled with (mean,variance) pairs and we assume $v = \kappa$ and $\gamma = 1$.}\label{fig:pra-counterexample2}
\end{figure}
%

